CTC Variations Through New WFST Topologies

This paper presents novel Weighted Finite-State Transducer (WFST) topologies to implement Connectionist Temporal Classification (CTC)-like algorithms for automatic speech recognition. Three new CTC variants are proposed: (1) the "compact-CTC", in which direct transitions between units are replaced with <epsilon> back-off transitions; (2) the "minimal-CTC", that only adds <blank> self-loops when used in WFST-composition; and (3) the "selfless-CTC" variants, which disallows self-loop for non-blank units. Compact-CTC allows for 1.5 times smaller WFST decoding graphs and reduces memory consumption by two times when training CTC models with the LF-MMI objective without hurting the recognition accuracy. Minimal-CTC reduces graph size and memory consumption by two and four times for the cost of a small accuracy drop. Using selfless-CTC can improve the accuracy for wide context window models.

==> topo_pics_src.tex <==
\def\greps{\detokenize{〈}\detokenize{ε}\detokenize{〉}}
\def\grblk{\detokenize{〈}b\detokenize{〉}}

\begin{figure*}[ht]
\vspace{-25pt} % adjust this
\hspace{-20pt} % adjust this
\minipage[t]{0.2\textwidth}
  \digraph[scale=0.5]{default2}{
    graph [fontname = "times" fontsize=18];
    node [fontname = "times" fontsize=18];
    edge [fontname = "times" fontsize=18];
	graph [label=<a) T.fst> labelloc=b center=1 nodesep=0.25 orientation=Portrait rankdir=LR ranksep=0.35 size="8.5,11"]
	0 [label=0 shape=doublecircle style=bold]
    0 -> 0 [label="\grblk:\greps"]
	1 [label=1 shape=doublecircle]
	0 -> 1 [label="A:A"]
	2 [label=2 shape=doublecircle]
	0 -> 2 [label="B:B"]
	1 -> 0 [label="\grblk:\greps"]
	1 -> 1 [label="A:\greps" style="dashed"]
	1 -> 2 [label="B:B"]
	2 -> 0 [label="\grblk:\greps"]
	2 -> 1 [label="A:A"]
	2 -> 2 [label="B:\greps" style="dashed"]
}
\label{fig:topologies_a}
\endminipage\hfill
\hspace{+17pt} % adjust this
\minipage[t]{0.2\textwidth}
  \digraph[scale=0.5]{eesen2}{
    graph [fontname = "times" fontsize=18];
    node [fontname = "times" fontsize=18];
    edge [fontname = "times" fontsize=18];
	graph [label=<b) T<SUB>eesen</SUB>.fst> labelloc=b center=1 nodesep=0.25 orientation=Portrait rankdir=LR ranksep=0.35 size="8.5,11"]
	0 [label=0 shape=doublecircle style=bold]
	1 [label=1 shape=circle]
	0 -> 1 [label="\greps:\greps"]
	1 -> 1 [label="\grblk:\greps"]
	3 [label=3 shape=circle]
	1 -> 3 [label="A:A"]
	4 [label=4 shape=circle]
	1 -> 4 [label="B:B"]
	2 [label=2 shape=circle]
	2 -> 0 [label="\greps:\greps"]
	2 -> 2 [label="\grblk:\greps"]
	3 -> 2 [label="\greps:\greps"]
	3 -> 3 [label="A:\greps" style="dashed"]
	4 -> 2 [label="\greps:\greps"]
	4 -> 4 [label="B:\greps" style="dashed"]
}
\label{fig:topologies_b}
\endminipage\hfill
\hspace{+65pt} % adjust this
\minipage[t]{0.2\textwidth}
  \digraph[scale=0.5]{compact2}{
    graph [fontname = "times" fontsize=18];
    node [fontname = "times" fontsize=18];
    edge [fontname = "times" fontsize=18];
	graph [label=<c) T<SUB>compact</SUB>.fst> labelloc=b center=1 nodesep=0.25 orientation=Portrait rankdir=LR ranksep=0.35 size="8.5,11"]
	0 [label=0 shape=doublecircle style=bold]
	0 -> 0 [label="\grblk:\greps"]
	1 [label=1 shape=circle]
	0 -> 1 [label="A:A"]
	2 [label=2 shape=circle]
	0 -> 2 [label="B:B"]
	1 -> 0 [label="\greps:\greps"]
	1 -> 1 [label="A:\greps" style="dashed"]
	2 -> 0 [label="\greps:\greps"]
	2 -> 2 [label="B:\greps" style="dashed"]
}
\label{fig:topologies_c}
\endminipage\hfill
\hspace{-56pt} % adjust this
\minipage[t]{0.2\textwidth}
  \digraph[scale=0.5]{minimal2}{
    graph [fontname = "times" fontsize=18];
    node [fontname = "times" fontsize=18];
    edge [fontname = "times" fontsize=18];
	graph [label=<d) T<SUB>minimal</SUB>.fst> labelloc=b center=1 nodesep=0.4 orientation=Portrait rankdir=LR ranksep=0.35 size="8.5,11"]
	0 [label=0 shape=doublecircle style=bold]
	0 -> 0 [label="\grblk:\greps" headport=e tailport=w]
	0 -> 0 [label="A:A" headport=e tailport=w]
	0 -> 0 [label="B:B" headport=e tailport=w]
}
\label{fig:topologies_d}
\endminipage
\hspace{-24pt} % adjust this
\vspace{-40pt} % adjust this
\caption{Example CTC topologies for a three-unit vocabulary: $\langle blank \rangle$, $A$, and $B$. Variants: a) correct-CTC, b) Eesen-CTC, c) compact-CTC, d) minimal-CTC. $\langle b \rangle$ states for $\langle blank \rangle$. Language unit-to-$\langle \epsilon \rangle$ selfloops are indicated by dashed arrows.}
\label{fig:topologies}
\vspace{-15pt} % adjust this
\end{figure*}

